ResQ: Mixed-Precision Quantization of Large Language Models with Low-Rank Residuals

Post-training quantization (PTQ) of large language models (LLMs) holds the promise in reducing the prohibitive computational cost at inference time. Quantization of all weight, activation and key-value (KV) cache tensors to 4-bit without significantly degrading generalizability is challenging, due to the high quantization error caused by extreme outliers in activations. To tackle this problem, we propose ResQ, a PTQ method that pushes further the state-of-the-art. By means of principal component analysis (PCA), it identifies a low-rank subspace (in practice 1/8 of the hidden dimension) in which activation variances are highest, and keep the coefficients within this subspace in high precision, e.g. 8-bit, while quantizing the rest to 4-bit. Within each subspace, invariant random rotation is applied to further suppress outliers. We show that this is a provably optimal mixed precision quantization scheme that minimizes error. With the Llama and Qwen2.5 families of models, we demonstrate that ResQ outperforms recent uniform and mixed precision PTQ methods on a variety of benchmarks, achieving up to 33\% lower perplexity on Wikitext than the next best method SpinQuant, and upto 3\times speedup over 16-bit baseline. Code is available at https://github.com/utkarsh-dmx/project-resq.

==> latex/Tables/generative_tasks_shortened.tex <==
\begin{table*}[]
\centering
\caption{Comparison of performance of quantization approaches on generative tasks at \textbf{W/A/KV = 4/4/4}. Our work ResQ and QUIK \cite{ashkboos2023quik} keep 12.5\% of channels in 8-bit.}
\label{tab:generative_benchmarks}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{c|c|c|cc|ccc}
\hline
 &  &  & \multicolumn{2}{c|}{\textbf{GSM8K 5-shot ($\uparrow$)}} & \multicolumn{3}{c}{\textbf{LongBench ($\uparrow$)}} \\ \cline{4-8}
\multirow{-2}{*}{\textbf{Model}} & \multirow{-2}{*}{\textbf{Method}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Training} \\ \textbf{Free}\end{tabular}} & flexible extract & strict match & qmsum & samsum & repobench-p \\ \hline \hline
 & 16-bit    & \cmark & 51.0 & 50.6 & 23.9 & 44.8 & 66.4 \\ \cdashline{2-8}
 & QUIK      & \cmark & 2.3  & 0.0  & 10.5 & 25.2 & 37.6 \\
 & QuaRot    & \cmark & 27.6 & 27.1 & 22.0 & 43.8 & 60.6 \\
 & SpinQuant & \xmark & 29.8 & 29.6 & 23.0 & 43.9 & \textbf{62.6} \\
\multirow{-5}{*}{Llama-3-8b} & \cellcolor[HTML]{CCFACC}ResQ  & \cellcolor[HTML]{CCFACC} \cmark& \cellcolor[HTML]{CCFACC}\textbf{33.6} & \cellcolor[HTML]{CCFACC}\textbf{33.2} & \cellcolor[HTML]{CCFACC}\textbf{23.1} & \cellcolor[HTML]{CCFACC}\textbf{44.1} & \cellcolor[HTML]{CCFACC}62.3 \\ \hline
 & 16-bit    & \cmark & 25.1 & 24.9 & 23.1 & 43.0 & 64.4 \\ \cdashline{2-8}
 & QUIK      & \cmark & 2.5  & 0.0  & 15.9 & 31.7 & 30.9 \\
 & QuaRot    & \cmark & 10.1 & 9.1 & 20.6 & 39.5 & 56.8 \\
 & SpinQuant & \xmark & 11.6 & 11.4 &   \textbf{21.7}   &  41.9    &   59.1   \\
\multirow{-5}{*}{Llama-3.2-3b} & \cellcolor[HTML]{CCFACC}ResQ & \cellcolor[HTML]{CCFACC} \cmark& \cellcolor[HTML]{CCFACC}\textbf{17.1} & \cellcolor[HTML]{CCFACC}\textbf{16.7} & \cellcolor[HTML]{CCFACC}\textbf{21.7} & \cellcolor[HTML]{CCFACC}\textbf{43.0} & \cellcolor[HTML]{CCFACC}\textbf{61.5} \\ \hline
\end{tabular}
}
\end{table*}
